PIAT: Parameter Interpolation based Adversarial Training for Image Classification

Adversarial training has been demonstrated to be the most effective approach to defend against adversarial attacks. However, existing adversarial training methods show apparent oscillations and overfitting issue in the training process, degrading the defense efficacy. In this work, we propose a novel framework, termed Parameter Interpolation based Adversarial Training (PIAT), that makes full use of the historical information during training. Specifically, at the end of each epoch, PIAT tunes the model parameters as the interpolation of the parameters of the previous and current epochs. Besides, we suggest to use the Normalized Mean Square Error (NMSE) to further improve the robustness by aligning the clean and adversarial examples. Compared with other regularization methods, NMSE focuses more on the relative magnitude of the logits rather than the absolute magnitude. Extensive experiments on several benchmark datasets and various networks show that our method could prominently improve the model robustness and reduce the generalization error. Moreover, our framework is general and could further boost the robust accuracy when combined with other adversarial training methods.

==> fig/CIFAR10_NMSE.tex <==
\begin{figure}
    \centering
    \subfigure[Hyperparameter analysis of $\mu$]{
    \includegraphics[width=9cm,height = 6.5cm]{fig/CIFAR10_NMSE.png}}
    \caption{Illustration of hyperparameter analysis of $\mu$. The different curve represents the accuracy under clean and different attack.
    }
    \label{fig:Hyperparameter Analysis}
\end{figure}

==> tab/MOMAT_WRN.tex <==
\begin{table*}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{c|c|cccccc}
\toprule
Dataset &Defense Method & NAT & PGD$^{20}$ & PGD$^{100}$ & MIM & CW & AA \\
\midrule
\multirow{6}{*}{CIFAR10}
&PGD-AT     & \textbf{86.87}& 48.77& 48.91&48.31&49.21&47.78\\
&TRADES($\beta=6$)    & 82.13& 55.14& 55.15 &55.19&52.56&50.38 \\
&MART  &84.26&54.11&54.13&55.20&53.41&50.20\\ 
&GAIRAT   &85.92&58.51&58.48&58.37&44.31&39.64\\ 
\cline{2-8}
&MOMAT+PGD-AT(Our)     & 85.56& \textbf{52.80}& \textbf{52.64}&\textbf{54.33}&\textbf{50.56}&\textbf{48.35}\\
%&MOMAT+TRADES(Our)     &82.08&58.93&85.94&59.27&55.15&53.73\\
&MOMAT+5NMSE &&&&&&\\ 
\midrule
\multirow{6}{*}{CIFAR100}
&PGD-AT    & 59.30& 28.13& 28.06 &28.95&27.01&23.99 \\
&TRADES ($\beta=6$) &&&&&&\\ 
&MART  &&&&&&\\ 
&GAIRAT   &&&&&&\\ 
%&TRADES($\beta=6$)    & 59.90& 29.84& 29.81 &30.32&27.27&25.42 \\
\cline{2-8}
&MOMAT+PGD-AT    & 60.09& 34.46& 34.41 &35.01&32.44&29.47     \\
%&MOMAT+TRADES($\beta=6$)    & 59.78& 34.52& 34.53 &34.99&30.69&29.25     \\
&MOMAT+5NMSE     & \textbf{61.04}& \textbf{35.15}& \textbf{35.19} &\textbf{35.72}&\textbf{32.69}&\textbf{30.07} \\
\midrule
\multirow{6}{*}{SVHN}
&PGD-AT    & \textbf{93.75}& \textbf{67.52}& \textbf{67.69} &\textbf{63.04}&\textbf{67.52}&36.64 \\
&TRADES ($\beta=6$) &&&&&&\\ 
&MART  &&&&&&\\ 
&GAIRAT   &&&&&&\\
\cline{2-8}
&MOMAT+PGD-AT &92.15&59.53&59.61&61.32&55.54&50.93 \\ 
&MOMAT+5NMSE    & 93.51& 65.76& 65.93 &65.39&62.61&\textbf{47.29} \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\centering
\end{table*}

==> tab/Parameter_NMSE.tex <==
\begin{table*}[!htp]
\caption{Combination of our framework using different hyperparameter in ResNet18 on CIFAR10.The maximum perturbation is $\boldsymbol{\epsilon} = \frac{8}{255}$. Average accuracy rates (\%) and results show that the MOMAT framework greatly improves the robustness of the model.}
\label{table 2: NMSE_table}
\centering
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{c|c|cccccc}
\toprule
Dataset &$\mu$ & NAT & PGD$^{20}$ & PGD$^{100}$ & MIM & CW & AA \\
\midrule
\multirow{9}*{CIFAF10}
%&PGD-AT    &84.28& 50.29& 50.12 &51.21&49.31&46.33 \\
%&PGD-AT+5NMSE    & 84.77& 51.56& 51.61 &52.98&50.94&46.60 \\
%&PGD-AT+10NMSE    & 83.95& 51.13&51.10 &52.84&50.63&46.68 \\
%&PGD-AT+15NMSE    & \textbf{84.88}&51.36&51.35&53.09&50.64&46.70 \\
%&PGD-AT+20NMSE    & 84.77&51.84&51.84&53.42&50.86&46.66 \\
&MOMAT &&&&&&\\ 
&MOMAT+3NMSE & 81.39& 53.36& 53.57 &54.49&51.70&48.62\\
&MOMAT+4NMSE    & 80.74& 53.45& 53.36 &54.22&51.38&48.69 \\
&MOMAT+5NMSE    & 80.76& \textbf{53.55}& 53.57 &\textbf{54.52}&51.47&48.70     \\
&MOMAT+6NMSE    & 80.76& 53.54& \textbf{53.59} &54.51&\textbf{51.72}&\textbf{48.80}     \\
\midrule
\multirow{8}*{CIFAF100}
%&PGD-AT    & 58.48& 28.36& 28.33 &29.30&27.06&23.85 \\
%&PGD-AT+5NMSE    & \textbf{58.88}& 29.55& 29.50 &30.47&28.18&24.82 \\
%&PGD-AT+10NMSE    & 57.75& 29.88&29.84 &30.54&27.71&24.75 \\
%&PGD-AT+15NMSE    & 58.32&29.31&29.33&30.22&27.58&24.40 \\
%&PGD-AT+20NMSE    & 57.60&29.23&29.24&30.21&27.72&24.67 \\
&MOMAT & 58.84& 29.11& 29.14 &29.97&27.89&24.15\\
&MOMAT+3NMSE &&&&&&\\
&MOMAT+4NMSE    & 54.35& 31.05& \textbf{31.01} &\textbf{31.49}&28.40&25.75 \\
&MOMAT+5NMSE    & 54.12& \textbf{31.11}& 30.99 &31.42&\textbf{28.45}&\textbf{25.79}     \\
&MOMAT+6NMSE &&&&&&\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\end{table*}

